Legal Case Document Summarization: Extractive and Abstractive Methods and their Evaluation

Summarization of legal case judgement documents is a challenging problem in Legal NLP. However, not much analyses exist on how different families of summarization models (e.g., extractive vs. abstractive) perform when applied to legal case documents. This question is particularly important since many recent transformer-based abstractive summarization models have restrictions on the number of input tokens, and legal documents are known to be very long. Also, it is an open question on how best to evaluate legal case document summarization systems. In this paper, we carry out extensive experiments with several extractive and abstractive summarization methods (both supervised and unsupervised) over three legal summarization datasets that we have developed. Our analyses, that includes evaluation by law practitioners, lead to several interesting insights on legal summarization in specific and long document summarization in general.

==> sections/abstractive.tex <==
\label{sec:abstr-impl}

Abstractive summarization methods have not been explored much in the legal domain.
A key challenge in applying such methods is that legal documents are usually very long, and most abstractive summarization models have restrictions on the number of input tokens.
%These methods generally consist of encoder-decoder architecture. They first try to encode the input into a hidden representation. Then depending upon the hidden representation, they generate the output summary. 
In this work, we apply several abstractive methods for legal document summarization, including both pretrained models and models finetuned for legal summarization. 
%We broadly classify the methods into the following five families -- Small, ExtAbs, Legal-pretrained, Legal-finetuned and Large. We first use the pretrained models from the families Small, ExtAbs, Legal-pretrained and Large. We then finetune the best performing models from Small, ExtAbs amd Legal-pretrained (to get Legal-finetuned). The idea behind using Legal-pretrained and Legal-finetuned models is to infuse legal domain knowledge. The Legal-pretrained models have a prior knolwedge of the legal language. 
%On top of that, we perform task-specific finetuning to get the Legal-finetuned model. We were not able to finetune methods from Large because of resource constraints. 

%(i)~\textbf{Small}: methods having a smaller input token limit and most applicable for summarizing shorter documents (e.g., news); (ii)~\textbf{ExtAbs}: abstractive summarization followed by extractive. (iii)~\textbf{Legal}: methods pretrained on legal corpora and (iv)~\textbf{Long}: methods designed to take as input longer documents (e.g., research and PubMed articles);From each family we pick representative methods, described below:

% We initially selected top-performing abstractive summarization algorithms from ~\cite{huang-etal-2020-achieved}. 

% (detailed subsequently in Section~\ref{ss:chunking}). 

% \textbf{(ii)~ExtAbs}: The previous approaches have difficulties in dealing with long documents due to the space complexity of the attention mechanism. 
% \todo{To balance the trade-off between input lengths that can be handled and the efficiency of the attention mechanism, some prior works have explored a hybrid of an abstractive and extractive approach~\cite{2step}.}
% \new{To balance the trade-off between input lengths that can be handled and the efficiency of the attention mechanism, we use a hybrid of an abstractive and extractive approach similar to ~\cite{2step}.}
% We experiment with such a hybrid approach combining pre-trained BERT extractive summarization and pre-trained BART abstractive summarization; we call this model BERT\_BART (details in Section~\ref{ss:extabs})

% \textbf{(iii)~Legal-pretrained}: While all the models stated above are pretrained on general text corpora, one way of incorporating domain knowledge into summarization is to pre-train models on domain-specific corpora.
% Among such methods, we experiment with legal-pegasus~\cite{legal-pegasus} which is pre-trained on legal data. Although trained on legal corpora, it has a restricted size, similar to the `Small' family. We show its applicability in Section~\ref{ss:chunking}.


% \textbf{(iv)~Legal-finetuned}: Another approach to incorporate domain knowledge is to apply task-specific finetuning to the models.  
% In this work, we attempt to  \textbf{finetune} some of the pre-trained models that perform the best.
% To this end, we have tried different ways of generating fine-tuning datasets; the details are in Section~\ref{sec:ft-abs}.
%by experimenting  with several similarity approaches. We also investigate the role of rhetorical labels for creating such datasets. 
%In this work, we attempt to \textbf{finetune} BART, BERT\_BART and Legal-Pegasus models, since these three perform the best among the pre-trained models.
%Note that we could not finetune Longformer with the resources available to us.

% \textbf{(v)~Large}: Some models have been recently developed for summarizing long document in a single step. 
% From this family of models, we investigate the Longformer~\cite{longformer}. Unlike the previous approaches, this model uses an attention mechanism capable of handling a large number of input tokens (details in Section~\ref{ss:long}).


% Finally, using ~\cite{divide&con}, we introduced rhetorical role labeling to split the document into segments and summarize each segment independently with a chunking-based fine-tuned BART model. 


\subsection{Pretrained Abstractive Models}
\label{sec:pretr-abs}


\subsubsection{Models meant for short documents}
\label{ss:chunking}

% From the `Small' family, we apply \textbf{Pointer Generator model (input token limit = 400)}~\footnote{https://github.com/abisee/pointer-generator} which is based on the sequence-to-sequence RNN paradigm that includes an encoder of bidirectional LSTM units and a unidirectional LSTM decoder. \textbf{BERTSum-Abs (512)}~\footnote{https://github.com/nlpyang/PreSumm} uses a modified BERT-based encoder and a 6-layer Transformer decoder with randomly initialized parameters. \textbf{BART (1024)}~\footnote{https://huggingface.co/facebook/bart-large} is a transformer-based sequence-to-sequence model pre-trained on a massive corpus of data using different strategies. \textbf{BigBird (4*1024)}~\footnote{\url{https://huggingface.co/google/bigbird-pegasus-large-pubmed}} is also a transformer-based model that uses a sparse attention mechanism, thus being able to support a larger input token limit.

These models have an input token limit which is usually shorter than the length of legal case documents. We apply the following models:
%(1)~\textbf{Pointer Generator}~\cite{see-etal-2017-get} (input token limit = 400) which is based on the sequence-to-sequence RNN paradigm that includes a BiLSTM encoder and a LSTM decoder. 
%(2)~\textbf{BERTSum-Abs}~\cite{DBLP:journals/corr/abs-1908-08345} (input token limit = 512) that uses a modified BERT-based encoder and a 6-layer Transformer decoder with randomly initialized parameters. 
(1)~\textbf{BART}~\cite{DBLP:journals/corr/abs-1910-13461} (input token limit = 1024), a pre-trained transformer-based Seq2Seq model. %pre-trained on a massive corpus of data using different strategies. 
%(4)~\textbf{BigBird}~\cite{zaheer2021big} (input token limit = 4*1024) that is also a transformer-based model that uses a sparse attention mechanism, thus being able to support a larger input token limit.
(2)~\textbf{Legal-Pegasus} (input token limit = 1024) which has a similar architecture like BART and is is already pretrained on legal documents. 
We use the implementations from the HuggingFace library (details in the Appendix).
We directly use their pre-trained versions to generate summaries of documents in the test sets. 

% The models have constraints on the input document length. They have a input token limit which is the number of tokens after which the document is truncated. As given in Table~\ref{tab:summ-dataset-stats}, legal documents are lengthier. Hence these methods cannot be used directly. We have replicated/reproduced these results using the \textit{chunking approach} 


\vspace{1mm}
\noindent \textbf{Challenges in using these models for summarizing legal case documents}: 
%The above models have shown success on various summarization datasets with short documents and short summaries (e.g., news articles). 
%Due to a huge number of words in documents and summaries in the legal datasets, there are some difficulties in applying some of these abstractive summarization models over long legal documents. 
The input token limit in these models is much smaller than the number of words in a typical  legal case document. 
Note that, by input token limit, we mean the number of tokens after which the documents are truncated while pre-training these models. 
This limit can theoretically be increased, %(e.g., we can use the Pointer Generator method with 20,000 as input token limit), 
but it would be practically infeasible because 
these methods have been designed and pre-trained for small input limits, and 
increasing the input limit would cause a considerable increase in the required GPU memory during task-specific fine-tuning (e.g., for BART, which we fine-tune later, the space required for the self-attention operation scales quadratically with the sequence length).
Hence, to apply these models on legal case documents, we apply a chunking-based approach as described below.

%These models are originally designed/pre-trained to take only a limited number of tokens in the input documents as shown in the table below. 

% \todo{abhay} ADD TABLE \\
% \begin{center}
% \begin{tabular}{|c | c|} 
%  \hline
%  Model & Input token limit  \\ [0.5ex] 
%  \hline
%  Pointer-Generator & 400 \\ 
%  \hline
%  BertSum-Abs & 512 \\
%  \hline
%  BART & 1024 \\
%  \hline
%  BigBird & 4*1024 \\
%  \hline
%  Longformer & 16*1024 \\
%  \hline
%  Pegasus & 512 \\ [1ex] 
%  \hline
% \end{tabular}
% \end{center}

\vspace{1mm}
\noindent \textbf{Chunking Approach}: 
%As a solution to the above problem, we take a chunking based approach. 
We first divide a document into small chunks, the size of each chunk being the maximum number of tokens (say, \textit{n}) that a model is designed/pre-trained to accept without truncating (e.g., $n=1024$ for BART). 
Specifically, the first \textit{n} tokens (without breaking sentences) go to the 1st chunk, the next \textit{n} tokens go to the 2nd chunk, and so on. 
Then we use a model to summarize every chunk. For a given document, we equally divide the target summary length among all the chunks. Finally, we append the generated summaries one after another. 
%Chunking is applied to methods from the `Small' and `Legal-pretrained' families.
%Note that, it is not possible to get gold-standard summaries for each individual chunk. 

%The size of each chunk is the maximum number of tokens that a model is designed for without truncating. For example, for BART, if the document has 1024*7 words, we will form 7 chunks of 1024 tokens.

%Although BigBird supports a larger chunksize, it cannot increase the input length limit up to our requirements. So we have used the chunking strategy but with a larger chunk size for BigBird.


%%%%%%%%%%%% commenting out from here %%%%%%%%%
\if 0

\vspace{1mm}
\noindent \textbf{Disadvantages of Chunking:} %Although using the chunking approach, we can handle long documents using the best short document summarization models; 
This chunking approach has two shortcomings: 
(1)~While summarizing, since we are only focusing upon a single chunk at a time, the contextual information from the remaining parts of the document is lost (i.e., there is no attention computed between chunks because the attention mechanism cannot operate across the boundaries of the chunks). 
To counter this limitation, models such as Longformer have been designed, as described below.
%While summarizing a chunk, the words/context in all the other chunks are not considered. 
(2)~An equal length summary is expected from each chunk, which is not an ideal approach, since some chunks can be more important than others. 
%A chunk may contribute more than the other chunks. 
For example, according to legal experts, the chunk containing the final judgment will contribute more to the summary than any other chunk.
One way to counter this limitation is to use a hybrid approach as described below.

\fi
%%%%%%%%%%%% commenting out till here %%%%%%%%%


\subsubsection{Models meant for long documents}
\label{ss:long}
%There is some information loss in both the above approaches. We therefore use Longformer~\cite{longformer} which has a higher input length capacity and can therefore handle the full document at once. 
Some models have been especially designed for handling long documents. We use the
Longformer~\cite{longformer} transformer architecture that uses sliding windows, dilated sliding windows, and global attention to achieve an attention mechanism that scales linearly with sequence length. 
%Although this attention mechanism can handle a large number of tokens, it does not consider attention score between every two tokens directly (unlike, say, BART and Pegasus). 
%This model compromises on attention scores to increase the input document token limit in this approach.
We use Legal-Longformer (Legal-LED: \url{https://huggingface.co/nsi319/legal-led-base-16384}) specifically finetuned on legal data. The model could accommodate the full legal case documents in most cases. Since a few documents in UK-Abs are longer (see Table ~\ref{tab:summ-dataset-stats}), those documents are truncated after 16,384 tokens. 
 


\subsubsection{Hybrid extractive-abstractive approach}
\label{ss:extabs}
% The previous approaches have difficulties in dealing with long documents due to the space complexity of the attention mechanism. To balance the trade-off between input lengths that can be handled and the efficiency of the attention mechanism, 
As mentioned earlier, to focus only on important parts of the document in the chunking-based approach,
we use a hybrid of an extractive approach and an abstractive approach, similar to~\cite{2step}. First, the document length is reduced by selecting salient sentences using a BERT-based extractive summarization model. 
Then a pre-trained BART model is used to generate the final summary~\cite{2step}. 
% Methods from  the ExtAbs family, which is a hybrid of abstractive and extractive summarization, can be used to counter this problem. 
% In this two-step approach introduced by~\cite{2step}, In the second step, an abstractive summarization model is used to generate the final summary.
%The original work~\cite{2step} used a pre-trained BART model to generate the final summary. 
Since, in our case, we often require a summary length greater than 1024 (see Table~\ref{tab:related-datasets}), we cannot directly use BART in the second step. 
Here we have two options -- either to use the a chunking-based BART summarization approach, or to use a pre-trained Longformer. 
Since the chunking-based BART summarization method performs better than the pre-trained Longformer (as we shall see later in Tables~\ref{tab:results-overall-in-ext}-~\ref{tab:results-overall-uk-abs}), we decided to use chunking-based BART in the second step.
We call this model BERT\_BART in the rest of the paper.

% Also, in this method, we use only pre-trained models. In the first step, we perform extractive summarization using pre-trained BERT to select salient sentences from the documents, and in the second step, we use chunking-based pre-trained BART summarization to get the final summary. 
% We call this model BERT\_BART.



\subsection{Finetuning Abstractive Models}
\label{sec:ft-abs}

Fine-Tuning transformer models has shown significant improvement in performance in most of the downstream tasks. Hence we try finetuning some of the abstractive models.
Our intention was to finetune some representative model from each of the 3 classes of models described in Section~\ref{sec:pretr-abs}.
%Transformer models like BART and Pegasus generally give significant improvements in summary after fine-tuning compared to pre-trained models. 
As we shall see later in Section~\ref{sec:results}, BART and Legal-Pegasus perform the best among the models meant for short documents. So we finetune the BART and  Legal-Pegasus models. 
We also use the finetuned BART as part of the BERT\_BART model.  
%We refer to this family of approaches as \textbf{Legal-finetuned.}
However, we could not finetune the Longformer model due to resource constraints.

\vspace{1mm}
\noindent {\bf Generating finetuning data:}
Finetuning summarization models needs a large set of document-summary pairs. 
However, as detailed in Sections~\ref{ss:chunking} and ~\ref{ss:extabs}, the models we finetune have a restricted input token limit which is lesser than the length of documents in our datasets. So, to generate the finetuning data for the chunking based summarization, we use the following method that is similar to the method in~\cite{divide&con}.

% Therefore, we use a chunking strategy for generating the finetuning data, which is similar to the method in~\cite{divide&con}.
%\new{The chunking strategy would not be necessary for fine-tuning Longformer, but because of resource constraints, that could not be attempted.}

Consider ($d$, $s$) to be a training document  and its reference (gold-standard) summary respectively. %point, where $d$ is the document and $s$ is its corresponding gold standard summary. 
When $d$ is segmented into $n$ chunks $d_1$, $d_2$, ... $d_n$, 
%the summary $s$ should also be segmented similarly, because 
it is not logical for the same $s$ to be the reference summary for each chunk $d_i$. 
What is desired is that every chunk $d_i$ has its \textit{chunked} reference summary $s_i$. %i.e., the finetuning data should consist of ($d_1$, $s_1$), ($d_2$, $s_2$) ... ($d_n$, $s_n$). 
%We call this data as \textit{finetuning data} in the rest of the paper.
%The fine-tuning data consists of chunks along with their summaries. The length of the chunk would depend on the model to be fine-tuned. The reference summaries for each chunk would be generated from the full document gold standard summary. 
We now discuss how we generate the summary $s_i$ for each chunk $d_i$.
%Initially, we consider both the document and summary as raw text. 
%To generate the summary $s_i$ for each chunk $d_i$, we use a sentence-by-sentence approach in which 
We first map every sentence in the full reference summary ($s$) to the most similar sentence in the input document. To this end, we use a variety of sentence-similarity measures, which we detail below.
Then for every chunk $d_i$, we combine all  sentences in $s$ which are mapped to any of the sentences in $d_i$, and consider those sentences as the summary $s_i$ (of $d_i$). 
%In the end, we also introduce a word threshold to ignore those chunks for which very short summaries are generated by this approach. 
Using the above method, from each document, we get a large number of ($d_i$, $s_i$) pairs which is used for finetuning. 

\vspace{1mm}
\noindent {\bf Sentence similarity measures:} The method for generating finetuning data  uses a similarity measure between two sentences (as stated above).
We experiment with three techniques for measuring sentence similarity between two sentences -- Mean Cosine Similarity (MCS), Smooth Inverse Frequency (SIF) and Cosine similarity with BERT [CLS] token (CLS-CS). Out of these, we find MCS to perform the best (Section~\ref{sec:results}). We describe MCS in detail here. Descriptions of SIF and CLS-CS can be found in the Appendix.
%Ranasinghe et al.~\cite{ranasinghe-etal-2019-enhancing} experimented with several sentence similarity techniques, out of which we experiment with two: 
%We use cosine similarity on average vector and cosine similarity using smooth inverse frequency from ~\cite{ranasinghe-etal-2019-enhancing}. We also use a rudimental approach considering only the [CLS] token encodings in the BERT embeddings. We generate three sets of fine-tuning data for each abstractive dataset using these similarity approaches.
%For measuring similarity, we have used the following three approaches.

In Mean Cosine Similarity (MCS)~\cite{ranasinghe-etal-2019-enhancing}, we first calculate the mean of BERT encodings of every token present in a sentence (using the SBERT model from ~\cite{reimers-2019-sentence-bert}) to get the encodings of the said sentence. 
Then we compute the cosine similarity between  the two sentence encodings.

% \textit{(ii) Smooth Inverse frequency with cosine similarity (SIF)}~\cite{ranasinghe-etal-2019-enhancing}: This approach is similar to the MCS approach; only here instead of mean, we consider a weighted mean, and we use a pre-trained BERT model. 
% The weight of every token $w$ is given by $\frac{a}{a + p(w)}$
% Where $p(w)$ is the estimated frequency of a word in the whole dataset.
% In other word, the weight for a word would be inversely proportional to the number of word occurrences. 
% %For the words like `is', `the', etc., the weight will be less and more importance would be given to the words occurring less.

% \textit{(iii) Cosine similarity with BERT [CLS] token (CLS-CS):} Here we consider the cosine similarity of the encodings of the CLS tokens of the two sentences (as given by the pre-trained BERT model). 

%We experimented with the different similarity approaches for creating finetuning data for BART --  BART\_CLS, BART\_MCS, BART\_SIF. As we shall find later in Section~\ref{sec:results}, MCS similarty performed the best. 



\vspace{2mm}
\noindent \textbf{Using Rhetorical Roles (RR) for generating finetuning data:} 
We also explore another method for generating finetuning data, that incorporates legal domain knowledge.
As described earlier in Section~\ref{sec:dataset}, a legal case document consists of 7 rhetorical segments such as Facts, Statutes, etc.
%Rhetorical role labels of sentences are  a source of legal domain knowledge. 
We incorporate this knowledge into our abstractive summarization process by combining it with the divide and conquer approach presented in~\cite{divide&con} (which is originally designed for summarizing research articles that are already segmented into logical segments). %Sentences in a legal case documents are not implicitly labelled with these roles. 

We first use a state-of-the-art classifier for rhetorical labeling of sentences in a legal document~\cite{deeprhole} to assign one of the labels -- RPC, FAC, STA, RLC, Ratio, PRE, ARG -- to each sentence of a document. 
We collate sentences of a particular role as one segment. Thus, effectively, we partition a document into 7 segments, each segment corresponding to a rhetorical role.
Then we apply the same approach as stated above to generate the summary of each segment; for this, we use the MCS sentence similarity measure (which performs the best, as we shall see later in Section~\ref{sec:results}). 
Note that, some of these rhetorical segments themselves may be longer than  the input token limit of BART and Pegasus; in such cases, we further divide the rhetorical segments into smaller chunks, and then generate the summary of each chunk. 
%We refer to this rhetorical role based finetuning strategy as BART\_MCS\_RR.
%In the end, we combine every segment summary according to a pre-defined order. For generating finetuning data, we first divided the documents into rhetorical role segments. 
%Since the length of some segments is still comparatively greater than the input token limit of BART and Pegasus, we apply the chunking-based approach here. Using the mean cosine similarity approach, we generate the reference summaries from the full document gold standard summaries for each chunk in each segment. 

\vspace{2mm}
\noindent 
We use all the methods stated above to generate fine-tuning datasets for IN-Abs and UK-Abs. First, using the three sentence similarity measures with the BART model, we generate BART\_CLS, BART\_MCS, BART\_SIF finetuned models. 
Out of these, BART\_MCS performs the best (as we will see in Section~\ref{sec:results}).
Therefore, we use MCS for generating finetuning data for the other models, to get Legal-Pegasus-MCS and BART\_MCS\_RR (where the finetuning data is generated based on rhetorical labels). 
We also use the finetuned BART\_MCS model with BERT\_BART method to get BERT\_BART\_MCS. 
Table~\ref{tab:hyp} gives the hyper-parameter details for finetuning the BART-based models and Legal-Pegasus.

We provide the URLs of the different pretrained abstractive models used in the paper and hyper-parameters for finetuning in the Appendix section of the paper.
% \begin{tabular}{|c | c| c| c|} 
%  \hline
%  Abs Algo & Sim Approach & Hyper-parameters  \\ [0.5ex] 
%  \hline
% BART & MCS &chunk size=1024, decoder max len = 512\\ 
%  \hline
 
%  \hline
% BART & SIF &chunk size=1024, p(w) from training data\\ 
%  \hline
 
%   \hline
% BART & CLS &chunk size=1024, decoder max len = 512\\ 
%  \hline
 
% Pegasus & MCS &chunk size=512, decoder max len = 256\\ 
%  \hline
 
%   BART & RR and MCS & chunk size=1024, decoder max len = 512\\ 
%  \hline

% \end{tabular}




%Using the above fine-tuning datasets, we fine-tuned BART and Pegasus models. We used 1024 chunk size for the BART model and 512 chunk size for the Pegasus model due to memory constraints. Table~\ref{tab:hyp} gives the hyper-parameter details.





% \todo{abhay} models not considering rhet role\\
% \todo{abhay} models considering rhet role


==> sections/extractive.tex <==
\label{sec:extr-impl}
There are four classes of methods that can be applied for extractive summarization of legal case documents.  We consider some representative methods from each class.

\subsection{Legal Domain-Specific Methods}

%The legal domain-specific methods can be further categorized into unsupervised (LetSum, KMM, CaseSummarizer and MMR) and supervised methods (Gist).

\subsubsection{Unsupervised:}  Among such methods, we reproduce the following four methods. 
\textbf{(1)~LetSum}~\cite{farzindar2004letsum} and \textbf{(2)~KMM}~\cite{farzindar2004letsum} -- both rank sentences based on term distribution models (TF-IDF and k-mixture model respectively). 
%As a post-processing step, the summaries are displayed in a structured way based on the rhetorical roles.
% Among such methods, we consider the following four as baselines -- \textbf{(1)~LetSum} and \textbf{(2)~KMM}: Both LetSum~\cite{farzindar2004letsum} and KMM~\cite{farzindar2004letsum} initially assigns rhetorical labels to sentences (using certain cue-phrases and CRF respectively). The sentences are ranked based on their TF-IDF values for LetSum and K-Mixture Model for KMM.  However, the rhetorical role information is {\it not} used for generating the summary. It acts as a {\it post-summarization step} that is mainly used for displaying the summary in a templatic/structured way. We therefore implement the sentence ranking modules for these baseline methods -- i.e, TF-IDF based summarization for LetSum and K-mixture model based summarization for KMM.
\textbf{(3)~CaseSummarizer}~\cite{polsley2016casesummarizer} ranks sentences based on their TF-IDF weights coupled with legal-specific features.
% with count of the number of legal terms (identified by a legal dictionary, ref. Section~\ref{sec:exp-setup}), statute terms, dates and named entities. \\
%The implementations and reproducibility challenges of the above methods are available in our prior work~\cite{bhattacharya2019comparative}.We newly reproduce/replicate the following methods in this paper:
\textbf{(4)~MMR}~\cite{zhong2019automatic} generates a template-based summary using a 2-stage classification framework and a Maximum Margin Relevance~\cite{zhong2019automatic} module.
% They experiment on  BVA decision of the US jurisdiction.
%In the absence of similar annotated training datasets to build a 2-stage classification framework for India and UK, we adopt only the Maximum Margin Relevance~\cite{zhong2019automatic} module of their work as a baseline. 
% containing (i) one sentence from the procedural history (ii) one sentence from issue (iii) one sentence from the service history of the veteran (iv) variable number of Reasoning \& Evidential Support sentences selected using Maximum Margin Relevance (v) one sentence from the conclusion. 
% Pattern-based regex extractors are used to identify the sentences (i)-(iii) and (v). Reasoning \& Evidential Support sentences are identified using Convolutional Neural Networks and summarized using Maximum Margin Relevance. The authors experiment on BVA decision of the US jurisdiction. In the absence of such annotated training datasets to build a 2-stage classification framework for India and UK, we adopt only the Maximum Margin Relevance~\cite{zhong2019automatic} module of their work as a baseline. 
%This method decides the inclusion of a sentence $s_i$ to the summary based on $\lambda \times Sim(s_i, \textit{Case}) + (1-\lambda) \times Sim(s_i, \textit{Summary})$, where \textit{Case} is the set of sentences in the original case document and \textit{Summary} represents the current set of sentences in the summary. $\lambda$ acts as the weight that balances the relevance and diversity; we consider $\lambda = 0.5$. 
%More elaborate information can be found in our Supplementary material.
Due to lack of space, reproducibility details of the above methods are given in the Appendix.

\subsubsection{Supervised:} 
To our knowledge, \textbf{Gist}~\cite{liu2019extracting} is the only supervised method specifically designed for summarizing legal case documents. We reproduce the method as its implementation is not publicly available. 
Gist first represents a sentence with different handcrafted features that are detailed in the Supplementary Information. 
%which includes the presence of specific legal terms. We use a legal dictionary mentioned in Section~\ref{sec:exp-setup}. 
The features include the word2vec embeddings of the sentence, for which we train a word2vec model on the training corpus ($7030$ documents of the IN-Abs and $693$ documents of the UK-Abs dataset). During evaluation, the trained word2vec model is used to derive the embeddings.

Based on the above features, Gist uses 3 models -- MLP, Gradient Boosted Decision Tree, LSTM -- to rank sentences in order of their likelihood to be included in the summary. We observe the best performance by using Gradient Boosted Decision Tree as the ML classifier, which we report. 

\subsection{Domain-independent methods}

%Domain-independent methods are those that can summarize \textit{any} document. We consider the following algorithms from this category:

\subsubsection{Unsupervised:} 
We consider the following popular algorithms from this class: \textbf{LexRank}~\cite{Erkan:2004},
\textbf{LSA}~\cite{Gong:2001},
\textbf{DSDR}~\cite{He-dsdr},
\textbf{Reduction}~\cite{jing2000sentence}.
We use the implementations from the Python~\textit{sumy} module for these methods. 
We also apply \textbf{PacSum}~\cite{pacsum}, a state-of-the-art method for unsupervised extractive summarization (implementation from~\url{https://github.com/mswellhao/PacSum}).

\subsubsection{Supervised:} Among these methods, we consider the neural methods \textbf{SummaRuNNer}~\cite{nallapati2017summarunner} (implementation available at \url{https://github.com/hpzhao/SummaRuNNer}) 
and \textbf{BERTSUM}~\cite{bertsum} (implementation available at \url{https://github.com/nlpyang/PreSumm}).\footnote{The original BERTSUM model uses a post-processing step called \textit{Trigram Blocking} that excludes a candidate sentence if it has a significant amount of trigram overlap with the already generated summary (to minimize redundancy in the summary). However, we observed that this step leads to summaries that are too short, as also observed in~\cite{ExtendedSumm}. Hence we ignore this step.}
Similar to Gist, these methods consider the task of extractive summarization as a binary classification problem.  The classifier returns a ranked list of sentences based on their prediction/confidence probabilities about their inclusion in the summary. We include sentences one-by-one from this list in decreasing order of their predicted probabilities into the summary, until the desired summary length is reached. 

%We also apply a recent BERT-based summarization method \textbf{BERTSUM}~\cite{bertsum} (implementation available at \url{https://github.com/nlpyang/PreSumm}). 
%In BERTSUM, the sentence selection function is a simple binary classification task (whether or not to include a sentence in the summary).\footnote{The original BERTSUM model uses a post-processing step called \textit{Trigram Blocking} that excludes a candidate sentence if it has a significant amount of trigram overlap with the already generated summary (to minimize redundancy in the summary). However, we observed that this step leads to summaries that are too short, as also observed in~\cite{ExtendedSumm}. Hence we ignore this step.} Similar to SummaRuNNer, we use the ranked list of sentences based on the confidence probabilities of their inclusion in the summary. We include sentences one-by-one into the final summary, until the desired length is reached.

\subsection{Training supervised extractive models}
\label{sub:train-data-supervised-extractive}

The supervised methods stated above (Gist, SumaRuNNer and BERTSUM) require labelled data for training, where every sentence in a training document must be labeled as $1$ if this sentence is suitable for inclusion in the summary, and labeled as $0$ otherwise.

As stated in Section~\ref{sec:dataset}, we use  parts of the IN-Abs and UK-Abs datasets for training supervised methods. 
%For the UK jurisdiction, we use a part of UK-Abs (for UK jurisdiction) for the training set. 
Since both these datasets have \textit{abstractive} summaries, they cannot be directly used to train extractive summarization methods. 
%Hence there is a necessity to convert the abstractive summaries to extractive for training such methods. 
We explore three methods -- Maximal, Avr and TF-IDF -- for converting the abstractive summaries to extractive for training such methods. We find that the performance of the supervised methods are better when the training data is generated through Avr, compared to the Maximal and TF-IDF methods. 
%Maximal is slow and computationally intensive and that it performs worse than Avr was also observed in~\cite{narayan2018ranking}. 
Hence we describe \textbf{Avr} in detail here and report results of the supervised methods where the training data is generated through \textbf{Avr}. Descriptions of Maximal and TF-IDF are stated in the Appendix.

% \textbf{(i)~Maximal}: In this approach proposed in~\cite{nallapati2017summarunner} the basic premise was to maximize the ROUGE score between the extractive and the abstractive gold-standard summaries. However global optimization is computationally expensive; a faster greedy strategy is -- keep adding sentences to the extractive summary one by one, each time selecting the sentence that when added to the already extracted summary has the maximum ROUGE score with respect to the abstractive gold-standard summary. 
%This process is repeated till the ROUGE score does not increase anymore. 
%Finally, all the sentences in this extractive summary are labelled as 1, the rest as 0.

\vspace{2mm}
\textbf{Avr}: We adopt the technique mentioned in~\cite{narayan2018ranking}.  For each sentence in the abstractive gold-standard summary, we select $3$ sentences from the source document (full text) that have the maximum average of ROUGE-1, ROUGE-2 and ROUGE-L scores w.r.t. the sentence in the abstractive summary. 
Then we take the union of all the sentences thus selected, and assign label them $1$ (to be included in the summary) and label other sentences in the source document as $0$. 

% \textbf{(iii)~TF-IDF}: 
%We calculated the TF-IDF vectors for all the sentences in the source document and those in the summary. 
%For each sentence in the summary, we find three sentences in the full text that are most similar to it. The similarity is measured as the cosine-similarity between the TF-IDF vectors of a sentence in the summary and a sentence in the source document, and similarity should be greater than $0.4$. 
%We label the sentences in the source document that are similar to some summary-sentence as 1, rest as 0.




==> sections/related_work.tex <==

Here we give a broad overview of some existing summarization algorithms (see~\cite{DBLP:journals/corr/abs-1804-04589,summarization-survey} for surveys).
%, both extractive and abstractive, legal domain specific and legal domain independent. 
Sections~\ref{sec:extr-impl} and ~\ref{sec:abstr-impl} give more details about the specific methods that we reproduce/replicate.

\noindent \textbf{Extractive Summarization Methods}: 
There is a wide variety of domain-independent (general) summarization methods. Unsupervised approaches range from graph-based~\cite{Erkan:2004,hiporank}, matrix factorization based~\cite{Gong:2001}, data reconstruction~\cite{He-dsdr} to recent BERT-based methods~\cite{pacsum}.
There are also many supervised neural text summarization models~\cite{nallapati2017summarunner,cheng2016neural,bertsum} which usually treat summarization as a classification problem (in-summary vs. out-of-summary). 
%Surveys of existing summarization methods can be found in~\cite{DBLP:journals/corr/abs-1804-04589,summarization-survey}.

Additionally, there are several domain-specific methods specifically developed for legal case document summarization.
There are several \textit{unsupervised} methods such as KMM~\cite{saravanan2006improving}, LetSum~\cite{farzindar2004letsum}, MMR~\cite{zhong2019automatic}, and CaseSummarizer~\cite{polsley2016casesummarizer}, %and DELSumm~\cite{delsumm}, 
and the supervised method Gist~\cite{liu2019extracting}. 
%is the only \textit{supervised} extractive method for legal case document summarization.
We reproduce all methods from this family. 
%except DELSumm, since, 
%unlike the other methods that take as input only a case document, DELSumm additionally requires a rhetorical label for each sentence in the document. 


%(iii)~Supervised, domain-independent: Given sufficient amount of training data, the methods can summarize documents of any kind~\cite{nallapati2017summarunner,cheng2016neural,bertsum}. We experiment with~\cite{nallapati2017summarunner} and ~\cite{bertsum}. A survey of the existing approaches can be found in~\cite{DBLP:journals/corr/abs-1804-04589}; (iv)~Supervised, domain-specific: To the best of our knowledge,Gist~\cite{liu2019extracting}. More details can be found in~\ref{sec:extr-impl}.

\noindent \textbf{Abstractive Summarization Methods}
The majority of the previous research on abstractive summarization deal with short documents to produce short summaries~\cite{see-etal-2017-get,DBLP:journals/corr/abs-1910-13461,DBLP:journals/corr/abs-1908-08345}. %~\cite{see-etal-2017-get}, ~\cite{DBLP:journals/corr/abs-1910-13461}, ~\cite{DBLP:journals/corr/abs-1908-08345}, ~\cite{DBLP:journals/corr/abs-1908-08345} are some of these methods/models/architectures which can be used to summarize short documents. 
A few studies~\cite{longformer,zaheer2021big} have introduced transformer architectures with a modified attention mechanisms which can be used for long document summarization. 
Bajaj et.al.~\cite{2step} developed a two-step approach for long document summarization -- they use a pre-trained BART model over compressed documents generated by identifying salient sentences. 
%They apply their method over a small set of legal documents with fewer words than our documents. 
In this work, we reproduce a simplified version of the method in~\cite{2step}. 
Gidiotis et.al.~\cite{divide&con} presents a divide and conquer approach for long document summarization, where they split the documents and summaries using sentence similarity into an ensemble of smaller summarization problems. 
In this work, we apply a method inspired from~\cite{divide&con} for finetuning and generating summaries using abstractive summarization models.

The only method for abstractive legal document summarization revealed by our literature search is LegalSumm~\cite{legalabs}. 
The method uses the RulingBR dataset (in Portugese language) which has  shorter documents and shorter summaries than the datasets considered in this work (see Table~\ref{tab:related-datasets}). 
A limitation of the method in~\cite{legalabs} is that it cannot generate summaries of more than 200 tokens, and hence this method cannot be directly applied to our datasets.
%Our experiments do not consider any such restriction. They also compare their method with two baseline approaches. In our work, we  report results of 11 abstractive methods (pretrained + finetuned).

\noindent \textbf{Differences with~\cite{bhattacharya2019comparative}}: 
Prior work by ~\cite{bhattacharya2019comparative} explored methods for legal document summarization. 
However there are several differences with this paper: 
(i)~The work mainly focused on extractive summarization and only the older abstractive Pointer-Generator model~\cite{pointer-generator}. Whereas, the present work explores a diverse set of abstractive summarization models including  transformer-based models.
(ii)~The present work explores several methods for creating training data for supervised extractive methods and finetuning data for supervised abstractive methods.
(iii)~While the prior work used only one dataset, here we experiment with three datasets from two different jurisdictions -- India and UK. 
%(ii)~We investigate several methods for creating training data to train supervised extractive methods; (iii)~We reproduce two more legal domain specific methods -- unsupervised MMR and supervised Gist; (iv)~We explore a diverse set of state-of-the-art abstractive summarization methods. We use pretrained models for generating summaries. Towards finetuning, we explore several training data generation strategies. 
In short, while ~\cite{bhattacharya2019comparative} was the first step, this paper takes a long leap in long legal document summarization.

==> sections/rhet-label.tex <==
Rhetorical role labelling of legal documents refer to the task of assigning semantic functions such as `Facts', `Arguments', `Final judgement', etc. to sentences in a judgement. It provides a structure to an otherwise unstructured, lengthy document. It enhances the readability of the case documents, e.g., a law practitioner may want to read only the facts or arguments of a case and also has potential applications in many downstream tasks including summarization.

Different prior works have considered different sets of rhetorical roles~\cite{farzindar2004letsum, saravanan2006improving,zhong2019automatic,bhattacharya2019identification}. 
It was shown in our prior work~\cite{bhattacharya2019comparative} that a mapping between the different sets of rhetorical roles is possible.  In this work, we consider a set of {\it seven} rhetorical roles suggested by the law experts whom we consulted. Briefly, the rhetorical roles are as follows --
\begin{enumerate}
    \item {\bf Facts (abbreviated as FAC)}: This refers to the chronology of events that led to filing the case, and how the case evolved over time in the legal system (e.g., First Information Report at a police station, filing an appeal to the Magistrate, etc.)  
    
    \item {\bf Ruling by Lower Court (RLC)}: Since we  are considering Supreme Court case documents, there were some judgements given by the lower courts (Trial Court, High Court, Tribunal, etc.) based on which the present appeal was made (to the Supreme Court). The verdict of the lower Court and the ratio behind the judgement by the lower Court was annotated with this label.

    \item {\bf Argument (ARG)}: The present Court's discussion on the law that is applicable to the set of proven facts by weighing the arguments of the contending parties.
    
    \item {\bf Statute (STA)}: Established laws referred to by the present court, which can come from a mixture of sources -- Acts , Sections, Articles, Rules, Order, Notices, Notifications, Quotations directly from the bare act, and so on.

    \item {\bf Precedent (PRE)}: Prior cases that were referred to, while arguing the present case. 

    \item {\bf Ratio of the decision (Ratio)}:   Application of the law along with reasoning/rationale on the points argued in the case; Reason given for the application of any legal principle to the legal issue.

    \item {\bf Ruling by Present Court (RPC)}: Ultimate decision / conclusion of the present Court following from the natural / logical outcome of the rationale.
    
\end{enumerate}

Towards automatating the task of rhetorical role labelling of a sentence in a case document, several models have been proposed. In our prior work~\cite{deeprhole}, we proposed several deep neural models for the task that was shown to give better performance than baseline methods. Specifically, Hier-BiLSTM-CRF performed best in rhetorical role labelling on documents from the Indian jurisdiction; LegalBert-BiLSTM-CRF performed best on documents from the UK jurisdiction. 

Some methods for summarization in this paper use the rhetorical role information of sentences as input for summarization (e.g. DELSumm for extractive and BART-MCS-RR for abstractive). These labels have been derived by the above models (Hier-BiLSTM-CRF for IN datasets and LegalBert-BiLSTM-CRF for UK dataset).
